New Quarkonium Results from the BABAR experiment

New BABAR results on B mesons and quarkonia are presented: an analysis of B+ --> X(3872)K+ and B0 --> X(3872)K0 decays with X(3872) --> J/Psi pi+pi-, a precise measurement of the B mass difference Delta mB = m(B0) - m(B+) and a study of hadronic transition between Upsilon mesons.

==> myDefinitions.tex <==
\RequirePackage{xspace}

\usepackage{relsize}

\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

\def\epem       {\ensuremath{e^+e^-}\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}

\def\B       {\ensuremath{B}\xspace}
\def\Bs       {\ensuremath{Bs}\xspace}
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}

\def\Xz  {\ensuremath{X(3872)}\xspace}

\def\q     {\ensuremath{q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}

\def\gaga  {\ensuremath{\gamma\gamma}\xspace}

\def\pion  {\ensuremath{\pi}\xspace}
\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pipi  {\ensuremath{\pip\pim}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kz   {\ensuremath{K^0}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 

\def\bone   {\ensuremath{b_1}\xspace}
\def\bonez  {\ensuremath{b_1^0}\xspace}
\def\bonep  {\ensuremath{b_1^+}\xspace}
\def\bonem  {\ensuremath{b_1^-}\xspace}
\def\bonemp {\ensuremath{b_1^\mp}\xspace}

\def\h     {\ensuremath{h}\xspace}
\def\hp   {\ensuremath{h^+}\xspace}
\def\hpm   {\ensuremath{h^\pm}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}

\def\Vud  {\ensuremath{V_{ud}}\xspace}
\def\Vtd  {\ensuremath{V_{td}}\xspace}
\def\Vub  {\ensuremath{V_{ub}}\xspace}
\def\Vtb  {\ensuremath{V_{tb}}\xspace}

\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}

\def\DeltaE     {\mbox{$\Delta E$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}

\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace} % no space before {...}!
\def\OneS{\Y1S}
\def\TwoS{\Y2S}
\def\ThreeS{\Y3S}
\def\FourS{\Y4S}
\def\NS{\ensuremath{\Upsilon{(nS)}}\xspace}
\def\MS{\ensuremath{\Upsilon{(mS)}}\xspace}
\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}

\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}

\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

\def\bxkch      {\ensuremath{\Bp \to \Xz \Kp}\xspace}
\def\bxkneu     {\ensuremath{\Bz \to \Xz \Kz}\xspace}
\def\bxk        {\ensuremath{\B \to \Xz \kaon}\xspace}
\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\xpsipipi {\ensuremath{\Xz \to \jpsi\pip\pim}}
\def\bpsipipik {\ensuremath{\Bpm \to \jpsi \pip \pim \Kpm}\xspace}

\def\bzpsikpi  {\ensuremath{\Bz \to \jpsi \Kp \pim}\xspace}
\def\bppsik    {\ensuremath{\Bp \to \jpsi \Kp}\xspace}
\def\bpsik    {\ensuremath{\B \to \jpsi \kaon}\xspace}

\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mum        {\ensuremath{\mu^-}\xspace}
\def\mumu       {\ensuremath{\mup\mum}\xspace}
\def\psimumu    {\ensuremath{\jpsi \to \mumu}\xspace}
\def\psiee    {\ensuremath{\jpsi \to \epem}\xspace}

\def\ep         {\ensuremath{e^+}\xspace}
\def\em            {\ensuremath{e^-}\xspace}
\def\epem         {\ensuremath{\ep\em}}
\def\psiee      {\ensuremath{\jpsi \to \epem}\xspace}

\def\YFourSetaYOneS {\ensuremath{\FourS \to \eta \OneS}\xspace}

\def\GG#1#2{\ensuremath{\Gamma(#1\to#2)\xspace}}

\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psitwospsipipi {\ensuremath{\psitwos \to \jpsi \pipi}\xspace}

\def\BR         {{\ensuremath{\cal B}\xspace}}

\def\etathreepi {\ensuremath{\eta \to \pipi\piz}\xspace}
\def\etagg {\ensuremath{\eta \to \gaga}\xspace}

\def\DISP{\displaystyle}

